Linear Partial Monitoring for Sequential Decision-Making: Algorithms, Regret Bounds and Applications

Partial monitoring is an expressive framework for sequential decision-making with an abundance of applications, including graph-structured and dueling bandits, dynamic pricing and transductive feedback models. We survey and extend recent results on the linear formulation of partial monitoring that naturally generalizes the standard linear bandit setting. The main result is that a single algorithm, information-directed sampling (IDS), is (nearly) worst-case rate optimal in all finite-action games. We present a simple and unified analysis of stochastic partial monitoring, and further extend the model to the contextual and kernelized setting.

==> parts/dueling-kernel.tex <==

\paragraph{Kernelized Dueling IDS}

Recall that  $\mathbf \by_t = [y_1, \dots, y_{t-1}]^\T$ is the vector that collects the observations and let $\{(a_s^1, a_s^2)\}_{s=1}^{t-1}$ be the action history. Note that for any $a \in \iI$ we can recover estimates for the utility  $g(a)$ via $\hat g_t(a) = \frac{1}{2} \hat f_t\big((a,a)\big)$. Using evaluation weights $k_t^g(a) \eqdef [k(a,a_s^1) - k(a,a_s^2)]_{s=1,\dots,t-1}$, we define the estimate
\begin{align}
	\hat g_t(a) = k_t^g(a)^\T (K_t  +\lambda \eye_{t-1})^{-1} \by_t\,. \label{eq:gallery-dueling-utility-estimate}
\end{align}
The maximizer of the estimated utility function is $\hat a_t = \argmax_{a \in \iI} \hat g_t(a)$. Note that the pair $(\hat a_t, \hat a_t) \in \aA$ is the greedy action for pair-wise evaluations.
%
%Then the least-squares solution $\hat f_t$ evaluated at any $x \in \xX$ is $\hat{f}_t(x) = k_t(x)^\T (K_t + \lambda \eye)^{-1} \mathbf \by_t$, where $\eye$ is the identity matrix in the appropriate dimension. To compute uncertainty estimates, we further define \todoj{regularizer}
%\begin{align*}
%	k_t(x,y) &\eqdef k(x,y) - k_t(x)^\T(K_t + \lambda\eye)^{-1}k_t(y)\,,\\
%	\sigma_t^2(x) &\eqdef k_t(x,x)\,.
%\end{align*} 
%For $\rho^2$-subgaussian dueling bandit feedback on reward functions with $\|f\|_{\hH} \leq B$, the \emph{confidence coefficient} is
%\begin{align*}
%	\beta_{t,\delta}^{1/2} &\eqdef \rho\sqrt{\log \det( \eye + \lambda^{-1} K_t)  + 2\log \tfrac{1}{\delta}} + \sqrt{\lambda}B\,.
%\end{align*}
%In particular, $\beta_{t,\delta}$ is defined such that the true function is in the \emph{confidence set} $\cC_t \eqdef \{ g \in \hH : \|g - \hat f_t\|_\hH^2 \leq \beta_{t, \delta}\} \subset \hH$ with high probability,
%\begin{align*}
%	\PP\left[\forall t \geq 1, f \in \cC_t \right] \geq 1 - \delta\,. 
%\end{align*}
%The confidence bound is by \citet[Theorem 3.11]{AbbasiYadkori2012}, which improves upon earlier results by \citet{Srinivas2009}.
%We use it to derive a bound on the estimated reward differences for all $x^1,x^2 \in \xX$, with probability at least $1-\delta$:\looseness=-1
%\begin{align*}
%	\left|\hat f_t(x^1) - \hat f_t(x^2) - \big(f(x^1) - f(x^2)\big)\right|^2 \leq \beta_{t,\delta} \psi_t(x^1, x^2)\,,
%\end{align*}
%where $\psi_t(x,z) \eqdef \sigma_t(x)^2 + \sigma_t(z)^2 - 2 k_t(x,z)$.
%
Define
\begin{align*}
	\delta_t &\eqdef \max_{b \in \iI} \hat g_t(b) - \hat g_t(\hat a_t) + (\beta_t \psi_t^g(b, \hat a_t))^{1/2}\,,
	%	\delta_t &\eqdef \max_{g \in \eE_t} \max_{b \in \iI} g(b) - g(\hat a_t)\\
	%	&= \max_{b \in \iI} \hat g_t(b) - \hat g_t(\hat a_t) + (\beta_t \psi_t^g(b, \hat a_t))^{1/2}\,,
\end{align*}
where we use $\beta_t = \beta_{t,1/t^2}$ as in \cref{lem:ls-kernel} and let $\psi_t^g(a,b) \eqdef \|k_a - k_b\|_{V_t^{-1}}^2$, which is computed with the kernel metric $\psi^g(a,b) \eqdef k(a,a) + k(b,b) - 2k(a,b)$ as follows:
\begin{align*}
	\psi_t^g(a,b) = \sdfrac{1}{\lambda}\big(\psi^g(a,b) - (k_t^g(a) - k_t^g(b))^\T (K_t + \lambda \eye_{t-1})^{-1} (k_t^g(a) - k_t^g(b))\big)\,.
\end{align*}
The gap estimate for the utility function is defined for any $a \in \iI$,
\begin{align}
	\hat \Delta_t^g(a) \eqdef \delta_t + \hat g_t(\hat a_t) - \hat g_t(a) \,, \label{eq:gallery-dueling-gap}
\end{align}
which is directly extended to pairs $\hat \Delta_t(a^1,a^2) \eqdef \hat \Delta_t^g(a^1) + \hat \Delta_t^g(a^2)$. Lastly, the information gain \cref{eq:kernel-info} for a pair of actions $(a^1,a^2)$ simplifies to
\begin{align}
	I_t(a^1, a^2) = \sdfrac{1}{2} \log\big(1 + \psi_t^g(a^1, a^2)\big)\,,\label{eq:gallery-dueling-info}
	%	&= \log \frac{\det (\eye + K_{t+1})}{\det (\eye + K_{t})} \nonumber
\end{align}

The key observation is that it suffices to optimize the information ratio over the set $\bB = \{(\hat a_t, b) : b \in \iI\}$. Note that $\bB$ contains the greedy action choice $(\hat a_t, \hat a_t)$ for which $I_t(\hat a_t, \hat a_t) = 0$. The approximate IDS algorithm restricted to the subset $\bB$  therefore randomizes between the greedy pair $(\hat a_t, \hat a_t)$ and some other action pair in $(\hat a_t,  b) \in \bB$, that provides information on the reward difference $g(\hat a_t) - g(b)$. Concretely, let 
\begin{align}
	c_t, p_t \eqdef \argmin_{c\in \iI,p \in [0,1]} \frac{\big((1-p) 2\delta_t + p (\delta_t + \hat \Delta_t^g(c))\big)^2}{pI_t(\hat a_t, c)}\,.
\end{align}
The trade-off probability $p_t(c)$ is obtained with \cref{lem:ratio-closed-form} in closed-form,
\[p_t(c) = \min\left(\frac{2\delta_t}{\hat \Delta_t^g(c) - \delta_t}, 1 \right)\,.\]
The approximate dueling policy then samples $a_t = (\hat a_t, \hat a_t)$ with probability $(1-p_t)$ and $a_t = (\hat a_t, c_t)$ with probability $p_t$. We denote the corresponding sampling distribution by $\muduel_t$.
To bound the information ratio for $\muduel_t$, we let $\bB_t^* = \{b \in \iI : \hat g_t(\hat a_t) - g(b) \leq (\beta_t \psi_t(b, \hat a_t))^{1/2}\}$. Note that 
\begin{align}
	\delta_t  &= \max_{b \in \iI} \hat g_t(b) - \hat g_t(\hat a_t) + (\beta_t \psi_t^g(b, \hat a_t))^{1/2} \nonumber\\
	&= \max_{b \in \bB_t^*} \hat g_t(b) - \hat g_t(\hat a_t) + (\beta_t \psi_t^g(b, \hat a_t))^{1/2} \nonumber\\
	&\leq \max_{b \in \bB_t^*} (\beta_t \psi_t^g(b, \hat a_t))^{1/2}\,.\label{eq:gallery-dueling-1}
\end{align}
The inequality follows by noting that $\hat g_t(b) \leq \hat g_t(\hat a_t)$ by definition of $\hat a_t$. The information-ratio is bounded by playing deterministically on $\bB_t^*$,
\begin{align*}
	\Psi_t(\muduel_t) = \frac{\hat \Delta_t(\muduel_t)^2}{I_t(\muduel_t)} &\leq \min_{b \in \bB_t^*} \frac{\hat \Delta_t(\hat a_t, b)^2}{I_t(\hat a_t, b)} = \min_{b \in \bB_t^*} \frac{(\delta_t +  \hDelta_t^g(b))^2}{I_t(\hat a_t, b)}\\
	&\leq \frac{9 \beta_t \psi_t(a_t, b)}{I_t(a_t, b)}\,.
\end{align*}
The second inequality follows from \cref{eq:gallery-dueling-1} and noting that any $b \in \bB_t^*$ satisfies $\hat \Delta_t^g(b) \leq (2 \beta_t \psi_t(b, \hat a_t))^{1/2}$. Lastly, assuming that the regularizer is chosen large enough such that $\psi_t(a,b) \leq 1$ holds for all $a,b \in \iI$, we get $I_t(\hat a_t,b) \geq 4 \psi_t(\hat a_t, b)$. Therefore, $\Psi_t(\muduel_t) \leq 36 \beta_t$. A regret bound for approximate dueling IDS follows with the established technique. The next corollary summarizes the result.
\begin{corollary}
	Assume that the feedback satisfies \cref{eq:gallery-dueling-feedback} for a function $g \in \hH(\iI)$ with bounded norm $\|g\|_\hH \leq B$ and $\rho$-sub-Gaussian observation noise. Then the regret of the dueling IDS (\cref{alg:ids-dueling}) satisfies
	\begin{align*}
		\R_n \leq \oO(\sqrt{n \beta_n \gamma_n})\,.
	\end{align*}
\end{corollary}
Using the same argument as in \cref{ss:linear-logarithmic} and assuming that the optimal action is unique, it is also possible to show a gap-dependent regret $\rR \leq \oO(\Delta_{\min}^{-1}\beta_n\gamma_n)$, where $\Delta_{\min}$ is the minimum gap of the utility function $g$. This translates to $\oO(\Delta_{\min}^{-1} d^2 \log(n)^2)$ regret for finite-dimensional parameter.

We remark that the worst-case analysis justifies the use of a deterministic action choice. The main difference is that the deterministic algorithm only chooses the greedy pair $(\hat a_t, \hat a_t)$ when $\delta_t = 0$, i.e.~when the optimal action has been identified with probability $1-t^{-2}$. On the other hand, the randomized IDS distribution samples the greedy pair as soon as $\delta_t \leq \hat \Delta_t^g(c_t)$.

The efficient version of IDS for dueling bandits is summarized in \cref{alg:ids-dueling}. In conclusion, by directly using the dueling structure, we reduced the computation complexity per round from $\oO(|\iI|^2)$ to $\oO(|\iI|)$, which makes the approach applicable to much larger actions. 








%Denote by $k_{t|a}$ and $\sigma_{t|a}$ the uncertainty estimates that are (tentatively) updated with an observation generated from $M_a$. Such an update does not require the observation outcome $y_t$, similar to the linear case, where we can update the precision matrix $V_{t|a} = V_t + M_a^\T M_a$. Further, let $w_{b,c} = \phi_b - \phi_c$ be the difference of kernel features for the gap difference that we want to estimate. The kernelized directed information gain is
%\begin{align*}
%	I_t(a;w_{b,c}) = \log \left(\frac{\sigma_t(b)^2 + \sigma_t(c)^2 - 2 k_t(b,c)}{\sigma_{t|a}(b)^2 + \sigma_{t|A_a}(c)^2 - 2 k_{t|a}(b,c)}\right)\,.
%\end{align*}
%As before the information processing inequality (Lemma \ref{lem:info-processing}) implies that $I_t(a;w_{b,c}) \leq I_t(a)$. \todoj{check this}



